A guide to mathematical quasicrystals

This introductory survey deals with mathematical and physical properties of discrete structures such as point sets and tilings. The emphasis is on proper generalizations of concepts and ideas from classical crystallography. In particular, we focus on their interplay with various physically motivated equivalence concepts such as local indistinguishability and local equivalence. Various discrete patterns with non-crystallographic symmetries are described in detail, and some of their magic properties are introduced. This perfectly ordered world is augmented by a brief introduction to the stochastic world of random tilings.

==> fontdef.tex <==
%                                                           fontdef.tex
% LaTeX NFSS font definition part for CM or PS fonts
% (c) Springer-Verlag HD
%----------------------------------------------------------------------
\if C\FONTS
%% This is file `fontdef.cm'
%% it is part of the Springer Verlag LaTeX support for use
%% with the New Font Selection Scheme.
%% From original copyright (C) 1989,1990 by Frank Mittelbach, Rainer Schoepf.
%% changed January 20th 1993 by Springer Verlag
%% It contains the NFSS-file 'fontdef.ori' with
%%
%% \def\fileversion{v1.1k}
%% \def\filedate{91/11/26}
%% \def\docdate {91/11/26}
%%
%% and only a few changes to the fonts that are selected.

%% Error Reports in case of UNCHANGED versions to
%%
%% Springer Verlag
%% Dept. New Technologies/Product Development
%% Tiergartenstrasse 17
%% D-W-6900 Heidelberg
%% FRG

\def\fileversion{v1.0}
\def\filedate{93/01/20}
\def\docdate {91/11/26}

%% \CheckSum{127}
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This file contains the external font information needed to load
%% the standard families of the computer modern fonts
%% designed by Donald E. Knuth.
%% This means that some of the font shapes are not available in
%% all sizes; in this case some other size (or other font) is
%% substituted instead.
%%
%% For a larger collection of fonts see the file `fontdef.max'.
%%
%% You should *not* change this file!  If you want to change the
%% fonts/shapes you should create a copy of it named `fontdef.tex'
%% and edit this one according to your needs!
%%
%% The format of a font/shape definition is as follows:
%%
%% \new@fontshape{family}{series}{shape}%
%%       {<size_1>external_font_1%
%%        <size_2>external_font_2%
%%        ...
%%        <size_n>external_font_n}{}
%%
%% (Don't forget the final {} !)
%%
%% family    : Name of font family like cmr etc.
%% series    : Weight and width of the font in 1 to 4 letter
%%             abbreviations. A table is given in the tugboat article
%%             distributed together with this file.
%% shape     : Either n (normal), it (italic), sc (small caps), sl
%%             (slanted) or u (upright italic).
%% <size_i>  : The size in printer points. Standard LaTeX supports 5,
%%             6, 7, 8, 9, 10, 11, 12, 14, 17, 20, 25 corresponding to
%%             \tiny, \scriptsize and so on.  The angle brackets are
%%             part of the syntax!
%%
%% external_font_i : The name of the external font in your font
%%             library. If the font/shape is not available in a
%%             certain size you may use the name of a replacement
%%             font.  E.g. one can substitute cmr5 for cmti.. which is
%%             only available in size 7 and higher.  If you put a `1'
%%             in front of the name of the font a warning message will
%%             be produced (saying that the font has been substituted
%%             for the real one) when you use it for the first time.
%%             Below you can find examples of this mechanism.
%%
%% For font/shape combinations which aren't available at all like
%% computer modern sans serif small caps a suitable default will be
%% used automatically unless you specify a substitution yourself with
%% the \subst@fontshape command.
%%
%% It syntax is as follows:
%%
%% \subst@fontshape{family}{series}{shape}%
%%                 {subst_family}{subst_series}{subst_shape}
%%
%% This might be necessary if the automatically selected default does
%% not match your needs. For example: the font shape choosen instead
%% of `computer modern sans serif small caps' would be `computer
%% modern sans serif normal'. With a \subst@fontshape command you can
%% change this, for example, to `computer modern roman small caps' as
%% we did below. (If you don't like this remove this line in your
%% *copy* of this file.)
%%
%% Finally, for every family there is an \extra@def macro.  It defines
%% special action to be done at load time for every font of the family.
%% In most cases you can simply write
%%
%% \extra@def{family}{}{}
%%
%% In this file it is used to suppress hyphenation for typewriter
%% fonts (see \extra@def{cmtt}... below) and to set the \skewchar
%% for math fonts (see \extra@def{cmm}... and \extra@def{cmsy}...).
%%
%%
\newlinechar`\^^J
\immediate\write\sixt@@n{File: `fontdef.cm' \space
 \fileversion\space <\filedate> (Springer Verlag)}
\immediate\write\sixt@@n{English Documentation
      \@spaces\space <\docdate> (FMi and RmS)}
\immediate\write\sixt@@n
  {^^JIncludes Font/Shape Definitions for:^^J
     ^^J\@spaces Computer Modern Standard Fonts%
  .^^J}
\immediate\write\sixt@@n
  {********************************************************************}
\immediate\write\sixt@@n
  {* Customized by Springer Verlag to change the default fonts.}
\immediate\write\sixt@@n
  {********************************************************************}
%%
%% Please don't change the next lines unless you know exactly what you
%% are doing.
%%
\def\default@shape{n}
\def\default@series{m}
\def\default@family{cmr}
\def\default@errfont{cmsy10}
%%
%% Again, this is doubly dangerous bent.
%%
\fontfamily\default@family
\fontseries\default@series
\fontshape\default@shape
%%
%% And here is your playground:
%%
\new@fontshape{cmr}{m}{n}{%
      <5>cmr5%
      <6>cmr6%
      <7>cmr7%
      <8>cmr8%
      <9>cmr9%
      <10>cmr10%
      <11>cmr10 at10.95pt%
      <12>cmr12%
      <14>cmr12 at14.4pt%
      <17>cmr17%
      <20>cmr17 at20.736pt%
      <25>cmr17 at24.8832pt}{}
\extra@def{cmr}{}{}
\new@fontshape{cmr}{m}{sl}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>cmsl8%
      <9>cmsl9%
      <10>cmsl10%
      <11>cmsl10 at10.95pt%
      <12>cmsl12%
      <14>cmsl12 at14.4pt%
      <17>cmsl12 at17.28pt%
      <20>cmsl12 at20.74pt%
      <25>cmsl12 at24.88pt%
      }{}

\new@fontshape{cmr}{m}{it}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>cmti7%
      <8>cmti8%
      <9>cmti9%
      <10>cmti10%
      <11>cmti10 at10.95pt%
      <12>cmti12%
      <14>cmti12 at14.4pt%
      <17>cmti12 at17.28pt%
      <20>cmti12 at20.74pt%
      <25>cmti12 at24.88pt%
      }{}

\new@fontshape{cmr}{m}{sc}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>cmcsc10 at8pt%
      <9>cmcsc10 at9pt%
      <10>cmcsc10%
      <11>cmcsc10 at10.95pt%
      <12>cmcsc10 at12pt%
      <14>cmcsc10 at14.4pt%
      <17>cmcsc10 at17.28pt%
      <20>cmcsc10 at20.74pt%
      <25>cmcsc10 at24.88pt%
      }{}
%%
%% Warning: please note that the upright shape below is used
%%          for the \pounds symbol of LaTeX. So this font
%%          definition shouldn't be removed.
%%
%          If cmu below 10pt is not available we substitute
%          cmti as far as possible (sizes 7, 8, 9). This is
%          done because cmu is used mainly for producing the
%          the \pound symbol and it is better to get a slanted
%          (or bigger) pound then to get a $ sign in such situations.
%%
\new@fontshape{cmr}{m}{u}{%
      <5>1cmti7%
      <6>1cmti7%
      <7>1cmti7%
      <8>1cmti8%
      <9>1cmti9%
      <10>cmu10%
      <11>cmu10 at10.95pt%
      <12>cmu10 at12pt%
      <14>cmu10 at14.4pt%
      <17>cmu10 at17.28pt%
      <20>cmu10 at20.74pt%
      <25>cmu10 at24.88pt%
      }{}

%%%%%%%% bold series

\new@fontshape{cmr}{b}{n}{%
      <5>1cmbx5%
      <6>1cmbx6%
      <7>1cmbx7%
      <8>1cmbx8%
      <9>1cmbx9%
      <10>cmb10%
      <11>cmb10 at10.95pt%
      <12>cmb10 at12pt%
      <14>cmb10 at14.4pt%
      <17>cmb10 at17.28pt%
      <20>cmb10 at20.736pt%
      <25>cmb10 at24.8832pt%
      }{}

%%%%%%%%% bold extended series

\new@fontshape{cmr}{bx}{n}{%
      <5>cmbx5%
      <6>cmbx6%
      <7>cmbx7%
      <8>cmbx8%
      <9>cmbx9%
      <10>cmbx10%
      <11>cmbx10 at10.95pt%
      <12>cmbx12%
      <14>cmbx12 at14.4pt%
      <17>cmbx12 at17.28pt%
      <20>cmbx12 at20.74pt%
      <25>cmbx12 at24.88pt%
      }{}

\new@fontshape{cmr}{bx}{sl}{%
      <5>1cmbx5%
      <6>1cmbx6%
      <7>1cmbx7%
      <8>1cmbx8%
      <9>1cmbx9%
      <10>cmbxsl10%
      <11>cmbxsl10 at10.95pt%
      <12>cmbxsl10 at12pt%
      <14>cmbxsl10 at14.4pt%
      <17>cmbxsl10 at17.28pt%
      <20>cmbxsl10 at20.74pt%
      <25>cmbxsl10 at24.88pt%
      }{}

\new@fontshape{cmr}{bx}{it}{%
      <5>1cmbx5%
      <6>1cmbx6%
      <7>1cmbx7%
      <8>1cmbx8%
      <9>1cmbx9%
      <10>cmbxti10%
      <11>cmbxti10 at10.95pt%
      <12>cmbxti10 at12pt%
      <14>cmbxti10 at14.4pt%
      <17>cmbxti10 at17.28pt%
      <20>cmbxti10 at20.74pt%
      <25>cmbxti10 at24.88pt%
      }{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Sans serif font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmss}{m}{n}{%
      <5>cmss10 at5pt%
      <6>cmss10 at6pt%
      <7>cmss10 at7pt%
      <8>cmss8%
      <9>cmss9%
      <10>cmss10%
      <11>cmss10 at10.95pt%
      <12>cmss12%
      <14>cmss12 at14.4pt%
      <17>cmss17%
      <20>cmss17 at20.74pt%
      <25>cmss17 at24.88pt%
      }{}


\subst@fontshape{cmss}{m}{it}{cmss}{m}{sl}

\new@fontshape{cmss}{m}{sl}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>cmssi8%
      <9>cmssi9%
      <10>cmssi10%
      <11>cmssi10 at10.95pt%
      <12>cmssi12%
      <14>cmssi12 at14.4pt%
      <17>cmssi17%
      <20>cmssi17 at20.74pt%
      <25>cmssi17 at24.88pt%
      }{}

%%%%%%% Font/shape undefined, therefore substituted

\subst@fontshape{cmss}{m}{sc}{cmr}{m}{sc}

%%%%%%%% semibold condensed series

\new@fontshape{cmss}{sbc}{n}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>1cmss8%
      <9>1cmss9%
       <10>cmssdc10%
       <11>cmssdc10 at10.95pt%
       <12>cmssdc10 at12pt%
       <14>cmssdc10 at14.4pt%
       <17>cmssdc10 at17.28pt%
       <20>cmssdc10 at20.74pt%
       <25>cmssdc10 at24.88pt%
       }{}

%%%%%%%%% bold extended series

\new@fontshape{cmss}{bx}{n}{%
      <5>1cmbx5%
      <6>1cmbx6%
      <7>1cmbx7%
      <8>1cmbx8%
      <9>1cmbx9%
      <10>cmssbx10%
      <11>cmssbx10 at10.95pt%
      <12>cmssbx10 at12pt%
      <14>cmssbx10 at14.4pt%
      <17>cmssbx10 at17.28pt%
      <20>cmssbx10 at20.74pt%
      <25>cmssbx10 at24.88pt%
      }{}

\extra@def{cmss}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Typewriter font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmtt}{m}{n}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>cmtt8%
      <9>cmtt9%
      <10>cmtt10%
      <11>cmtt10 at10.95pt%
      <12>cmtt12%
      <14>cmtt12 at14.4pt%
      <17>cmtt12 at17.28pt%
      <20>cmtt12 at20.74pt%
      <25>cmtt12 at24.88pt%
      }{}

\new@fontshape{cmtt}{m}{it}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>1cmtt8%
      <9>1cmtt9%
      <10>cmitt10%
      <11>cmitt10 at10.95pt%
      <12>cmitt10 at12pt%
      <14>cmitt10 at14.4pt%
      <17>cmitt10 at17.28pt%
      <20>cmitt10 at20.74pt%
      <25>cmitt10 at24.88pt%
      }{}

\new@fontshape{cmtt}{m}{sl}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>1cmtt8%
      <9>1cmtt9%
      <10>cmsltt10%
      <11>cmsltt10 at10.95pt%
      <12>cmsltt10 at12pt%
      <14>cmsltt10 at14.4pt%
      <17>cmsltt10 at17.28pt%
      <20>cmsltt10 at20.74pt%
      <25>cmsltt10 at24.88pt%
      }{}

\new@fontshape{cmtt}{m}{sc}{%
      <5>1cmr5%
      <6>1cmr6%
      <7>1cmr7%
      <8>1cmtt8%
      <9>1cmtt9%
      <10>cmtcsc10%
      <11>cmtcsc10 at10.95pt%
      <12>cmtcsc10 at12pt%
      <14>cmtcsc10 at14.4pt%
      <17>cmtcsc10 at17.28pt%
      <20>cmtcsc10 at20.74pt%
      <25>cmtcsc10 at24.88pt%
      }{}

\extra@def{cmtt}{\hyphenchar #1\m@ne}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Math italic font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmm}{m}{it}{%
      <5>cmmi5%
      <6>cmmi6%
      <7>cmmi7%
      <8>cmmi8%
      <9>cmmi9%
      <10>cmmi10%
      <11>cmmi10 at10.95pt%
      <12>cmmi12%
      <14>cmmi12 at14.4pt%
      <17>cmmi12 at17.28pt%
      <20>cmmi12 at20.74pt%
      <25>cmmi12 at24.88pt%
      }{}

\new@fontshape{cmm}{b}{it}{%
      <5>cmmib10 at5pt%
      <6>cmmib10 at6pt% 1cmmi6%
      <7>cmmib10 at7pt%
      <8>cmmib10 at8pt% 1cmmi8%
      <9>cmmib10 at9pt% 1cmmi9%
      <10>cmmib10%
      <11>cmmib10 at10.95pt%
      <12>cmmib10 at12pt%
      <14>cmmib10 at14.4pt%
      <17>cmmib10 at17.28pt%
      <20>cmmib10 at20.74pt%
      <25>cmmib10 at24.88pt%
      }{}

\extra@def{cmm}{\skewchar#1'177}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Math symbol font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmsy}{m}{n}{%
      <5>cmsy5%
      <6>cmsy6%
      <7>cmsy7%
      <8>cmsy8%
      <9>cmsy9%
      <10>cmsy10%
      <11>cmsy10 at10.95pt%
      <12>cmsy10 at12pt%
      <14>cmsy10 at14.4pt%
      <17>cmsy10 at17.28pt%
      <20>cmsy10 at20.74pt%
      <25>cmsy10 at24.88pt%
      }{}

\new@fontshape{cmsy}{b}{n}{%
      <5>cmbsy10 at5pt%
      <6>cmbsy10 at6pt%
      <7>cmbsy10 at7pt%
      <8>cmbsy10 at8pt%
      <9>cmbsy10 at9pt%
      <10>cmbsy10%
      <11>cmbsy10 at10.95pt%
      <12>cmbsy10 at12pt%
      <14>cmbsy10 at14.4pt%
      <17>cmbsy10 at17.28pt%
      <20>cmbsy10 at20.74pt%
      <25>cmbsy10 at24.88pt%
      }{}

\extra@def{cmsy}{\skewchar#1'60}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  LaTeX symbol font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{lasy}{m}{n}{%
      <5>lasy5%
      <6>lasy6%
      <7>lasy7%
      <8>lasy8%
      <9>lasy9%
      <10>lasy10%
      <11>lasy10 at10.95pt%
      <12>lasy10 at12pt%
      <14>lasy10 at14.4pt%
      <17>lasy10 at17.28pt%
      <20>lasy10 at20.74pt%
      <25>lasy10 at24.88pt%
      }{}

\new@fontshape{lasy}{b}{n}{%
      <5>lasyb10 at5pt%
      <6>lasyb10 at6pt%
      <7>lasyb10 at7pt%
      <8>lasyb10 at8pt%
      <9>lasyb10 at9pt%
      <10>lasyb10%
      <11>lasyb10 at10.95pt%
      <12>lasyb10 at12pt%
      <14>lasyb10 at14.4pt%
      <17>lasyb10 at17.28pt%
      <20>lasyb10 at20.74pt%
      <25>lasyb10 at24.88pt%
      }{}

\extra@def{lasy}{}{}
\else

%%
%% This is file `fontdef.ps'
%% it is part of the Springer Verlag LaTeX support for use
%% with the New Font Selection Scheme.
%% From original copyright (C) 1989,1990 by Frank Mittelbach, Rainer Schoepf.
%% changed January 20th 1993 by Springer Verlag
%%
%% It provides font selection including PostScript fonts
%% using the NFSS from Frank Mittelbach, Rainer Schoepf.

%% Error Reports in case of UNCHANGED versions to
%%
%% Springer Verlag
%% Dept. New Technologies/Product Development
%% Tiergartenstrasse 17
%% D-W-6900 Heidelberg
%% FRG

\def\fileversion{v1.0}
\def\filedate{93/01/20}

%% \CheckSum{126}
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This file contains the external font information needed to load
%% the standard families of the computer modern fonts
%% designed by Donald E. Knuth.
%% This means that some of the font shapes are not available in
%% all sizes; in this case some other size (or other font) is
%% substituted instead.
%%
%% For a larger collection of fonts see the file `fontdef.max'.
%%
%% You should *not* change this file!  If you want to change the
%% fonts/shapes you should create a copy of it named `fontdef.tex'
%% and edit this one according to your needs!
%%
%% The format of a font/shape definition is as follows:
%%
%% \new@fontshape{family}{series}{shape}%
%%       {<size_1>external_font_1%
%%        <size_2>external_font_2%
%%        ...
%%        <size_n>external_font_n}{}
%%
%% (Don't forget the final {} !)
%%
%% family    : Name of font family like cmr etc.
%% series    : Weight and width of the font in 1 to 4 letter
%%             abbreviations. A table is given in the tugboat article
%%             distributed together with this file.
%% shape     : Either n (normal), it (italic), sc (small caps), sl
%%             (slanted) or u (upright italic).
%% <size_i>  : The size in printer points. Standard LaTeX supports 5,
%%             6, 7, 8, 9, 10, 11, 12, 14, 17, 20, 25 corresponding to
%%             \tiny, \scriptsize and so on.  The angle brackets are
%%             part of the syntax!
%%
%% external_font_i : The name of the external font in your font
%%             library. If the font/shape is not available in a
%%             certain size you may use the name of a replacement
%%             font.  E.g. one can substitute cmr5 for cmti.. which is
%%             only available in size 7 and higher.  If you put a `1'
%%             in front of the name of the font a warning message will
%%             be produced (saying that the font has been substituted
%%             for the real one) when you use it for the first time.
%%             Below you can find examples of this mechanism.
%%
%% For font/shape combinations which aren't available at all like
%% computer modern sans serif small caps a suitable default will be
%% used automatically unless you specify a substitution yourself with
%% the \subst@fontshape command.
%%
%% It syntax is as follows:
%%
%% \subst@fontshape{family}{series}{shape}%
%%                 {subst_family}{subst_series}{subst_shape}
%%
%% This might be necessary if the automatically selected default does
%% not match your needs. For example: the font shape choosen instead
%% of `computer modern sans serif small caps' would be `computer
%% modern sans serif normal'. With a \subst@fontshape command you can
%% change this, for example, to `computer modern roman small caps' as
%% we did below. (If you don't like this remove this line in your
%% *copy* of this file.)
%%
%% Finally, for every family there is an \extra@def macro.  It defines
%% special action to be done at load time for every font of the family.
%% In most cases you can simply write
%%
%% \extra@def{family}{}{}
%%
%% In this file it is used to suppress hyphenation for typewriter
%% fonts (see \extra@def{cmtt}... below) and to set the \skewchar
%% for math fonts (see \extra@def{cmm}... and \extra@def{cmsy}...).
%%
%%
\newlinechar`\^^J
\immediate\write\sixt@@n{File: `fontdef.ps' \space
 \fileversion\space <\filedate> (Springer Verlag)}
\immediate\write\sixt@@n
  {********************************************************************}
\immediate\write\sixt@@n
  {*by Springer Verlag from M & S original, to support PostScript fonts *}
\immediate\write\sixt@@n
  {********************************************************************}
%%
%% Please don't change the next lines unless you know exactly what you
%% are doing.
%%
\def\default@shape{n}
\def\default@series{m}
\def\default@family{cmr}
\def\default@errfont{cmsy10}
%%
%% Again, this is doubly dangerous bent.
%%
\family\default@family
\series\default@series
\shape\default@shape
%%
%% And here is your playground:
%%
%%
%% Generalized scheme for PostScript fonts, assuming they
%% all have the same basic structure
\def\postscript@fontdef#1#2#3#4#5#6#7#8{
% 1 : full name for family
% 2 : short name for family
% 3 : tfm name for normal font
% 4 : tfm name for italic font
% 5 : tfm name for bold font
% 6 : tfm name for bolditalic font
% 7 : tfm name for smallcaps font
% 8 : tfm name for slanted font
\immediate\write\sixt@@n
  {********************************************************************}
\immediate\write\sixt@@n
  {Defining fonts for PostScript #1 family, with }
\immediate\write\sixt@@n
  {#2 as shortname}
\immediate\write\sixt@@n
  {#3 as TFM name for normal font}
\immediate\write\sixt@@n
  {#4 as TFM name for italic font}
\immediate\write\sixt@@n
  {#5 as TFM name for bold font}
\immediate\write\sixt@@n
  {#6 as TFM name for bolditalic font}
\immediate\write\sixt@@n
  {#7 as TFM name for smallcaps font}
\immediate\write\sixt@@n
  {#8 as TFM name for slanted font}

\immediate\write\sixt@@n
  {********************************************************************}
\new@fontshape{#2}{m}{n}{%
      <5>#3 at5pt%
      <6>#3 at6pt%
      <7>#3 at7pt%
      <8>#3 at8pt%
      <9>#3 at9pt%
      <10>#3 at10pt%
      <11>#3 at11pt%
      <12>#3 at12pt%
      <14>#3 at14pt%
      <17>#3 at17pt%
      <20>#3 at20pt%
      <25>#3 at25pt}{}
\extra@def{#2}{}{}

\new@fontshape{#2}{m}{sc}{%
      <5>#7 at5pt%
      <6>#7 at6pt%
      <7>#7 at7pt%
      <8>#7 at8pt%
      <9>#7 at9pt%
      <10>#7 at10pt%
      <11>#7 at11pt%
      <12>#7 at12pt%
      <14>#7 at14pt%
      <17>#7 at17pt%
      <20>#7 at20pt%
      <25>#7 at25pt%
      }{}


\new@fontshape{#2}{m}{it}{%
      <5>#4 at5pt%
      <6>#4 at6pt%
      <7>#4 at7pt%
      <8>#4 at8pt%
      <9>#4 at9pt%
      <10>#4 at10pt%
      <11>#4 at11pt%
      <12>#4 at12pt%
      <14>#4 at14pt%
      <17>#4 at17pt%
      <20>#4 at20pt%
      <25>#4 at25pt%
      }{}

\new@fontshape{#2}{m}{sl}{%
      <5>#8 at5pt%
      <6>#8 at6pt%
      <7>#8 at7pt%
      <8>#8 at8pt%
      <9>#8 at9pt%
      <10>#8 at10pt%
      <11>#8 at11pt%
      <12>#8 at12pt%
      <14>#8 at14pt%
      <17>#8 at17pt%
      <20>#8 at20pt%
      <25>#8 at25pt%
      }{}

\new@fontshape{#2}{bx}{n}{%
      <5>#5 at6pt%
      <6>#5 at6pt%
      <7>#5 at7pt%
      <8>#5 at8pt%
      <9>#5 at9pt%
      <10>#5 at10pt%
      <11>#5 at11pt%
      <12>#5 at12pt%
      <14>#5 at14pt%
      <17>#5 at17pt%
      <20>#5 at20pt%
      <25>#5 at25pt%
      }{}

\new@fontshape{#2}{bx}{it}{%
      <5>#6 at6pt%
      <6>#6 at6pt%
      <7>#6 at7pt%
      <8>#6 at8pt%
      <9>#6 at9pt%
      <10>#6 at10pt%
      <11>#6 at11pt%
      <12>#6 at12pt%
      <14>#6 at14pt%
      <17>#6 at17pt%
      <20>#6 at20pt%
      <25>#6 at25pt%
      }{}


% bold and bold-extended regarded as the same
% slanted and smallcaps only in normal font
\subst@fontshape{#2}{b}{sc}{#2}{m}{sc}
\subst@fontshape{#2}{b}{sl}{#2}{m}{sl}
\subst@fontshape{#2}{bx}{sc}{#2}{m}{sc}
\subst@fontshape{#2}{bx}{sl}{#2}{m}{sl}
\subst@fontshape{#2}{b}{n}{#2}{bx}{n}
\subst@fontshape{#2}{b}{it}{#2}{bx}{it}
}
%%
%\new@fontshape{cmr}{m}{n}{%
%      <5>cmr5%
%      <6>cmr6%
%      <7>cmr7%
%      <8>cmr8%
%      <9>cmr9%
%      <10>cmr10%
%      <11>cmr10 at10.95pt%
%      <12>cmr12%
%      <14>cmr12 at14.4pt%
%      <17>cmr17%
%      <20>cmr17 at20.736pt%
%      <25>cmr17 at24.8832pt}{}
%\extra@def{cmr}{}{}
%\new@fontshape{cmr}{m}{sl}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>cmsl8%
%      <9>cmsl9%
%      <10>cmsl10%
%      <11>cmsl10 at10.95pt%
%      <12>cmsl12%
%      <14>cmsl12 at14.4pt%
%      <17>cmsl12 at17.28pt%
%      <20>cmsl12 at20.74pt%
%      <25>cmsl12 at24.88pt%
%      }{}
%
%\new@fontshape{cmr}{m}{it}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>cmti7%
%      <8>cmti8%
%      <9>cmti9%
%      <10>cmti10%
%      <11>cmti10 at10.95pt%
%      <12>cmti12%
%      <14>cmti12 at14.4pt%
%      <17>cmti12 at17.28pt%
%      <20>cmti12 at20.74pt%
%      <25>cmti12 at24.88pt%
%      }{}
%
%\new@fontshape{cmr}{m}{sc}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>cmcsc10 at8pt%
%      <9>cmcsc10 at9pt%
%      <10>cmcsc10%
%      <11>cmcsc10 at10.95pt%
%      <12>cmcsc10 at12pt%
%      <14>cmcsc10 at14.4pt%
%      <17>cmcsc10 at17.28pt%
%      <20>cmcsc10 at20.74pt%
%      <25>cmcsc10 at24.88pt%
%      }{}
%%%
%%% Warning: please note that the upright shape below is used
%%%          for the \pounds symbol of LaTeX. So this font
%%%          definition shouldn't be removed.
%%%
%%          If cmu below 10pt is not available we substitute
%%          cmti as far as possible (sizes 7, 8, 9). This is
%%          done because cmu is used mainly for producing the
%%          the \pound symbol and it is better to get a slanted
%%          (or bigger) pound then to get a $ sign in such situations.
%%%
%\new@fontshape{cmr}{m}{u}{%
%      <5>1cmti7%
%      <6>1cmti7%
%      <7>1cmti7%
%      <8>1cmti8%
%      <9>1cmti9%
%      <10>cmu10%
%      <11>cmu10 at10.95pt%
%      <12>cmu10 at12pt%
%      <14>cmu10 at14.4pt%
%      <17>cmu10 at17.28pt%
%      <20>cmu10 at20.74pt%
%      <25>cmu10 at24.88pt%
%      }{}
%
%%%%%%%%% bold series
%
%\new@fontshape{cmr}{b}{n}{%
%      <5>1cmbx5%
%      <6>1cmbx6%
%      <7>1cmbx7%
%      <8>1cmbx8%
%      <9>1cmbx9%
%      <10>cmb10%
%      <11>cmb10 at10.95pt%
%      <12>cmb10 at12pt%
%      <14>cmb10 at14.4pt%
%      <17>cmb10 at17.28pt%
%      <20>cmb10 at20.736pt%
%      <25>cmb10 at24.8832pt%
%      }{}
%
%%%%%%%%%% bold extended series
%
%\new@fontshape{cmr}{bx}{n}{%
%      <5>cmbx5%
%      <6>cmbx6%
%      <7>cmbx7%
%      <8>cmbx8%
%      <9>cmbx9%
%      <10>cmbx10%
%      <11>cmbx10 at10.95pt%
%      <12>cmbx12%
%      <14>cmbx12 at14.4pt%
%      <17>cmbx12 at17.28pt%
%      <20>cmbx12 at20.74pt%
%      <25>cmbx12 at24.88pt%
%      }{}
%
%\new@fontshape{cmr}{bx}{sl}{%
%      <5>1cmbx5%
%      <6>1cmbx6%
%      <7>1cmbx7%
%      <8>1cmbx8%
%      <9>1cmbx9%
%      <10>cmbxsl10%
%      <11>cmbxsl10 at10.95pt%
%      <12>cmbxsl10 at12pt%
%      <14>cmbxsl10 at14.4pt%
%      <17>cmbxsl10 at17.28pt%
%      <20>cmbxsl10 at20.74pt%
%      <25>cmbxsl10 at24.88pt%
%      }{}
%
%\new@fontshape{cmr}{bx}{it}{%
%      <5>1cmbx5%
%      <6>1cmbx6%
%      <7>1cmbx7%
%      <8>1cmbx8%
%      <9>1cmbx9%
%      <10>cmbxti10%
%      <11>cmbxti10 at10.95pt%
%      <12>cmbxti10 at12pt%
%      <14>cmbxti10 at14.4pt%
%      <17>cmbxti10 at17.28pt%
%      <20>cmbxti10 at20.74pt%
%      <25>cmbxti10 at24.88pt%
%      }{}

\postscript@fontdef{Times}{cmr}{psmtimr}{psmtimi}{psmtimb}%
{psmtimbi}{cmcsc10}{psmtimi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Sans serif font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\postscript@fontdef{Helvetica}{cmss}{psmhlv}{psmhlvo}{psmhlvb}%
{psmhlvbo}{psmhlv}{psmhlv}

%\new@fontshape{cmss}{m}{n}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>cmss8%
%      <9>cmss9%
%      <10>cmss10%
%      <11>cmss10 at10.95pt%
%      <12>cmss12%
%      <14>cmss12 at14.4pt%
%      <17>cmss17%
%      <20>cmss17 at20.74pt%
%      <25>cmss17 at24.88pt%
%      }{}
%
%
%\subst@fontshape{cmss}{m}{it}{cmss}{m}{sl}
%
%\new@fontshape{cmss}{m}{sl}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>cmssi8%
%      <9>cmssi9%
%      <10>cmssi10%
%      <11>cmssi10 at10.95pt%
%      <12>cmssi12%
%      <14>cmssi12 at14.4pt%
%      <17>cmssi17%
%      <20>cmssi17 at20.74pt%
%      <25>cmssi17 at24.88pt%
%      }{}
%
%%%%%%%% Font/shape undefined, therefore substituted
%
%\subst@fontshape{cmss}{m}{sc}{cmr}{m}{sc}
%
%%%%%%%%% semibold condensed series
%
%\new@fontshape{cmss}{sbc}{n}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>1cmss8%
%      <9>1cmss9%
%       <10>cmssdc10%
%       <11>cmssdc10 at10.95pt%
%       <12>cmssdc10 at12pt%
%       <14>cmssdc10 at14.4pt%
%       <17>cmssdc10 at17.28pt%
%       <20>cmssdc10 at20.74pt%
%       <25>cmssdc10 at24.88pt%
%       }{}
%
%%%%%%%%%% bold extended series
%
%\new@fontshape{cmss}{bx}{n}{%
%      <5>1cmbx5%
%      <6>1cmbx6%
%      <7>1cmbx7%
%      <8>1cmbx8%
%      <9>1cmbx9%
%      <10>cmssbx10%
%      <11>cmssbx10 at10.95pt%
%      <12>cmssbx10 at12pt%
%      <14>cmssbx10 at14.4pt%
%      <17>cmssbx10 at17.28pt%
%      <20>cmssbx10 at20.74pt%
%      <25>cmssbx10 at24.88pt%
%      }{}
%
%\extra@def{cmss}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Typewriter font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\postscript@fontdef{Courier}{cmtt}{psmcou}{psmcouo}{psmcoub}%
{psmcoubo}{psmcou}{psmcou}
\extra@def{cmtt}{\hyphenchar #1\m@ne}{}

%\new@fontshape{cmtt}{m}{n}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>cmtt8%
%      <9>cmtt9%
%      <10>cmtt10%
%      <11>cmtt10 at10.95pt%
%      <12>cmtt12%
%      <14>cmtt12 at14.4pt%
%      <17>cmtt12 at17.28pt%
%      <20>cmtt12 at20.74pt%
%      <25>cmtt12 at24.88pt%
%      }{}
%
%\new@fontshape{cmtt}{m}{it}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>1cmtt8%
%      <9>1cmtt9%
%      <10>cmitt10%
%      <11>cmitt10 at10.95pt%
%      <12>cmitt10 at12pt%
%      <14>cmitt10 at14.4pt%
%      <17>cmitt10 at17.28pt%
%      <20>cmitt10 at20.74pt%
%      <25>cmitt10 at24.88pt%
%      }{}
%
%\new@fontshape{cmtt}{m}{sl}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>1cmtt8%
%      <9>1cmtt9%
%      <10>cmsltt10%
%      <11>cmsltt10 at10.95pt%
%      <12>cmsltt10 at12pt%
%      <14>cmsltt10 at14.4pt%
%      <17>cmsltt10 at17.28pt%
%      <20>cmsltt10 at20.74pt%
%      <25>cmsltt10 at24.88pt%
%      }{}
%
%\new@fontshape{cmtt}{m}{sc}{%
%      <5>1cmr5%
%      <6>1cmr6%
%      <7>1cmr7%
%      <8>1cmtt8%
%      <9>1cmtt9%
%      <10>cmtcsc10%
%      <11>cmtcsc10 at10.95pt%
%      <12>cmtcsc10 at12pt%
%      <14>cmtcsc10 at14.4pt%
%      <17>cmtcsc10 at17.28pt%
%      <20>cmtcsc10 at20.74pt%
%      <25>cmtcsc10 at24.88pt%
%      }{}
%
%\extra@def{cmtt}{\hyphenchar #1\m@ne}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Math italic font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmm}{m}{it}{%
      <5>cmmi5%
      <6>cmmi6%
      <7>cmmi7%
      <8>cmmi8%
      <9>cmmi9%
      <10>cmmi10%
      <11>cmmi10 at10.95pt%
      <12>cmmi12%
      <14>cmmi12 at14.4pt%
      <17>cmmi12 at17.28pt%
      <20>cmmi12 at20.74pt%
      <25>cmmi12 at24.88pt%
      }{}

\new@fontshape{cmm}{b}{it}{%
      <5>cmmib10 at5pt%<5>1cmmi5%
      <6>cmmib10 at6pt%<6>1cmmi6%
      <7>cmmib10 at7pt%<7>1cmmi7%
      <8>cmmib10 at8pt%<8>1cmmi8%
      <9>cmmib10 at9pt%<9>1cmmi9%
      <10>cmmib10%
      <11>cmmib10 at10.95pt%
      <12>cmmib10 at12pt%
      <14>cmmib10 at14.4pt%
      <17>cmmib10 at17.28pt%
      <20>cmmib10 at20.74pt%
      <25>cmmib10 at24.88pt%
      }{}

\extra@def{cmm}{\skewchar#1'177}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Math symbol font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{cmsy}{m}{n}{%
      <5>cmsy5%
      <6>cmsy6%
      <7>cmsy7%
      <8>cmsy8%
      <9>cmsy9%
      <10>cmsy10%
      <11>cmsy10 at10.95pt%
      <12>cmsy10 at12pt%
      <14>cmsy10 at14.4pt%
      <17>cmsy10 at17.28pt%
      <20>cmsy10 at20.74pt%
      <25>cmsy10 at24.88pt%
      }{}

\new@fontshape{cmsy}{b}{n}{%
      <5>cmbsy10 at5pt%<5>1cmsy5%
      <6>cmbsy10 at6pt%<6>1cmsy6%
      <7>cmbsy10 at7pt%<7>1cmsy7%
      <8>cmbsy10 at8pt%<8>1cmsy8%
      <9>cmbsy10 at9pt%<9>1cmsy9%
      <10>cmbsy10%
      <11>cmbsy10 at10.95pt%
      <12>cmbsy10 at12pt%
      <14>cmbsy10 at14.4pt%
      <17>cmbsy10 at17.28pt%
      <20>cmbsy10 at20.74pt%
      <25>cmbsy10 at24.88pt%
      }{}

\extra@def{cmsy}{\skewchar#1'60}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  LaTeX symbol font shapes
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{lasy}{m}{n}{%
      <5>lasy5%
      <6>lasy6%
      <7>lasy7%
      <8>lasy8%
      <9>lasy9%
      <10>lasy10%
      <11>lasy10 at10.95pt%
      <12>lasy10 at12pt%
      <14>lasy10 at14.4pt%
      <17>lasy10 at17.28pt%
      <20>lasy10 at20.74pt%
      <25>lasy10 at24.88pt%
      }{}

\new@fontshape{lasy}{b}{n}{%
      <5>lasyb10 at5pt%<5>1lasy5%
      <6>lasyb10 at6pt%<6>1lasy6%
      <7>lasyb10 at7pt%<7>1lasy7%
      <8>lasyb10 at8pt%<8>1lasy8%
      <9>lasyb10 at9pt%<9>1lasy9%
      <10>lasyb10%
      <11>lasyb10 at10.95pt%
      <12>lasyb10 at12pt%
      <14>lasyb10 at14.4pt%
      <17>lasyb10 at17.28pt%
      <20>lasyb10 at20.74pt%
      <25>lasyb10 at24.88pt%
      }{}

\extra@def{lasy}{}{}





%%
%% End of file `fontdef.ps'.



\fi
\endinput


==> preload.tex <==
%% Save file as: PRELOAD.MIN            Source: FILESERV@SHSU.BITNET
%% Note: This is a file from the FONTSEL set written by Frank Mittelbach
%%       <PZF5HZ@RUIPC1E.BITNET> and Rainer Schoepf <SCHOEPF@SC.ZIB-Berlin.DE>
%%
%% This is file `/usr2/distrib/latex209/nfss/preload.min' generated
%% on <1991/11/22> with the docstrip utility (v1.1k).
%%
%% The original source files were:
%%
%% preload.doc  (with modules: `min')

%%
%% Copyright (C) 1989,1990,1991 by Frank Mittelbach, Rainer Schoepf.
%% All rights reserved.
%%
%% This file is part of the NFSS (New Font Selection Scheme) package.
%%
%% IMPORTANT NOTICE:
%%
%% You are not allowed to change this file. You may however copy this file
%% to a file with a different name and then change the copy if you obey
%% the restrictions on file changes described in readme.mz.
%%
%% You are allowed to distribute this file under the condition that it is
%% distributed together with all files mentioned in readme.mz3. If you
%% receive only some of these files from someone, complain!
%%
%% You are NOT ALLOWED to distribute this file alone. You are NOT ALLOWED
%% to take money for the distribution or use of either this file or a
%% changed version, except for a nominal charge for copying etc.
%%
%% For error reports in case of UNCHANGED versions see readme files.
%%
%% Please do not request updates from us directly. Distribution is done
%% through Mail-Servers and TeX organizations.
%%

\def\fileversion{v1.0h}
\def\filedate{91/11/22}
\def\docdate {91/11/22}

%% \CheckSum{52}
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}

%%
%% This file preloads the absolute minimum of fonts (5) needed
%% to successfully generate a format file for LaTeX.
%%
%% You should *not* change this file!  If you want to preload more
%% or less fonts you should create a copy of it named `preload.tex'
%% and edit this one according to your needs!
%%
%%
\immediate\write\sixt@@n{File: `preload.%
 min' \space
 \fileversion\space <\filedate> (FMi and RmS)}
\immediate\write\sixt@@n{English Documentation
     \@spaces\space  <\docdate> (FMi and RmS)}
\immediate\write\sixt@@n
  {********************************************************************}
\immediate\write\sixt@@n
  {* Probably customized by YOU who forgot to change the lines above! *}
\immediate\write\sixt@@n
  {********************************************************************}
%%
%%    We begin by loading the math extension font (cmex10)
%%    and the \LaTeX{} line and circle fonts.
%%    It is necessary to do this explicitly since these are
%%    used by {\tt lplain.tex} and {\tt latex.tex}.
%%    Since the internal font name contains \verb+/+ characters
%%    and digits we construct the name via \verb+\csname+.
\expandafter\font\csname cmex/m/n/10\endcsname=cmex10
\font\tenln  =line10   \font\tenlnw  =linew10
\font\tencirc=lcircle10 \font\tencircw=lcirclew10

%% The preloads below (with comment signs in front) will be loaded
%% whenever standard \LaTeX{} is starting in 10pt size. So maybe you
%% like to preload at least these 9 fonts or a similar set if you
%% prefer documents in 11pt or 12pt size.

%%%%%%%%%%%%%%%%%%%%%%%%%
%% cm roman fonts
%%%%%%%%%%%%%%%%%%%%%%%%%

 %% None preloaded
 %% \preload@sizes{cmr}{m}{n}{5,7,10}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% cm sans serif fonts
%%%%%%%%%%%%%%%%%%%%%%%%%

 %% None preloaded

%%%%%%%%%%%%%%%%%%%%%%%%%
%% cm typewriter fonts
%%%%%%%%%%%%%%%%%%%%%%%%%

 %% None preloaded

%%%%%%%%%%%%%%%%%%%%%%%%%
%% cm math fonts
%%%%%%%%%%%%%%%%%%%%%%%%%

 %% \preload@sizes{cmm}{m}{it}{5,7,10}
 %% \preload@sizes{cmsy}{m}{n}{5,7,10}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% LaTeX symbol fonts
%%%%%%%%%%%%%%%%%%%%%%%%%

 %% None preloaded


\endinput
%%
%% End of file `/usr2/distrib/latex209/nfss/preload.min'.

